On Properties of Policy-Based Specifications

The advent of large-scale, complex computing systems has dramatically increased the difficulties of securing accesses to systems' resources. To ensure confidentiality and integrity, the exploitation of access control mechanisms has thus become a crucial issue in the design of modern computing systems. Among the different access control approaches proposed in the last decades, the policy-based one permits to capture, by resorting to the concept of attribute, all systems' security-relevant information and to be, at the same time, sufficiently flexible and expressive to represent the other approaches. In this paper, we move a step further to understand the effectiveness of policy-based specifications by studying how they permit to enforce traditional security properties. To support system designers in developing and maintaining policy-based specifications, we formalise also some relevant properties regarding the structure of policies. By means of a case study from the banking domain, we present real instances of such properties and outline an approach towards their automatised verification.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{M.H. ter Beek and A. Lluch Lafuente (Eds.): 11th International Workshop\\
on Automated Specification and Verification of Web Systems (WWV'15).\\
EPTCS 188, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.188.5}{10.4204/EPTCS.188.5}}

